FLAME: Factuality-Aware Alignment for Large Language Models

Alignment is a standard procedure to fine-tune pre-trained large language models (LLMs) to follow natural language instructions and serve as helpful AI assistants. We have observed, however, that the conventional alignment process fails to enhance the factual accuracy of LLMs, and often leads to the generation of more false facts (i.e. hallucination). In this paper, we study how to make the LLM alignment process more factual, by first identifying factors that lead to hallucination in both alignment steps:\ supervised fine-tuning (SFT) and reinforcement learning (RL). In particular, we find that training the LLM on new knowledge or unfamiliar texts can encourage hallucination. This makes SFT less factual as it trains on human labeled data that may be novel to the LLM. Furthermore, reward functions used in standard RL can also encourage hallucination, because it guides the LLM to provide more helpful responses on a diverse set of instructions, often preferring longer and more detailed responses. Based on these observations, we propose factuality-aware alignment, comprised of factuality-aware SFT and factuality-aware RL through direct preference optimization. Experiments show that our proposed factuality-aware alignment guides LLMs to output more factual responses while maintaining instruction-following capability.

==> Factuality-Aware_Alignment_For_Large_Language_Models/bio_gen_exp.tex <==
\begin{table}[t!]
	\caption{Pilot study on biography generation. Pos. denotes the positives for SFT or DPO. Neg. denotes the negatives for DPO. FS denotes FActScore.}
	\label{tb:pilot_study_bio_gen}
	\centering
	 \resizebox{1\columnwidth}{!}{  
   \begin{threeparttable}
	  % \setlength\tabcolsep{0.2cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 7B}& \multicolumn{2}{c|}{src. of supervision}& \multicolumn{2}{c}{\textbf{Bio}} \\
\cmidrule(rl){2-3} \cmidrule(rl){4-5} 
 & Pos.& Neg.& FS& \# Corr. / Err.\\
 \hline
 % (1)& Chat version&	32.4&	21.3&	43.4 \\
 (1) \pt& -& -&	39.1&	14.4 / 22.0\\
 (2) \ragpt& -& -&55.4&	18.6 / 15.9\\
 \hline
(3) \multirow{2}{*}{\sft} & \pt& -&	37.9&	13.4 / 21.8\\
(4) & \ragpt& -&	35.7&	13.5 / 23.7\\
 \hline
(5) \multirow{2}{*}{\dpo} & \pt\tnote{$\ast$}& \pt\tnote{$\ast$}&	41.6&	15.4 / 20.7\\
(6) & \ragpt& \pt&	23.5& 12.7 / 34.9\\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
 		\begin{tablenotes}
	\item[$\ast$] FActScore is used to select positives and negatives. 
    \end{tablenotes}
    \end{threeparttable}
	}
 \vspace{-0.4cm}
\end{table}


==> Factuality-Aware_Alignment_For_Large_Language_Models/dpo_ablation.tex <==
\begin{table}[t]
	\caption{Ablation on factuality preference data creation.}
	\label{tb:dpo_ablations}
	\centering
	 \resizebox{1\columnwidth}{!}{  
\begin{threeparttable}
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{ccc|c|c}
\hline \hline
\multicolumn{3}{c|}{Factuality preference data}&\multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{1}{c}{\textbf{\textbf{Bio}}}\\
 \cmidrule(rl){1-3} \cmidrule(rl){4-4} \cmidrule(rl){5-5}
Reward model& Pos.,Neg.& \# pairs& win rate\tnote{$\triangle$}& FS\\
\hline
\factrm& max, min& 3,315& 51.7& 44.9\\
\factrm& enum.& 5,126& 50.7& 45.0\\
\selfrm\ + $5*$\factrm& max, min& 6,340& 50.1& 45.1 \\
\hline \hline
	\end{tabular}
 \begin{tablenotes}
        \item[$\triangle$] comparing with DPO baseline, \sft{} + \dpo. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality-Aware_Alignment_For_Large_Language_Models/dpo_exp.tex <==
\begin{table*}[t!]
\caption{Experiments of direct preference optimization (DPO). IF.~and Fact.~denote instruction following $(x, y_{+}, y_{-})$ and factuality $(x \in X^{\text{\tiny fact}}, y_{\text{\tiny true}}, y_{\text{\tiny false}})$ preference data, where $X^{\text{\tiny fact}}$ denotes the set of fact-based instructions. \factonlydpo{} denotes the variant which only optimizes factuality. The preference data statistics is listed in Appendix, Table~\ref{tb:training_data_statistics}.}
	\label{tb:main_dpo_results}
	\centering
	 \resizebox{1\textwidth}{!}{  
	  % \setlength\tabcolsep{0.15cm}
    \begin{tabular}{l|cc|c|cc|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 70B} & \multicolumn{2}{c|}{src. of supervision}& \multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{Bio}}& \multicolumn{2}{c}{\textbf{Alpaca Fact}}& \multicolumn{2}{c}{\textbf{FAVA}}\\
 \cmidrule(rl){2-3} \cmidrule(rl){4-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(rl){9-10}
 & IF.& Fact.& win rate over  (2)& FS& \# Corr. / Err.& FS& \# Corr. / Err.& FS& \# Corr. / Err.\\
 \hline
 (0) Chat& \multicolumn{2}{c|}{Proprietary data}& 66.2& 33.2& 23.4 / 43.6& 39.3& 22.3 / 36.4& 47.5& 28.0 / 31.3\\
 \hline
 (1) \sft& -& -& 27.1& 44.7& 21.1 / 26.8& 38.6& 16.7 / 29.0& 54.4& 21.2 / 25.8\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
(2) + \dpo& \checkmark& \xmark& 50.0& 42.3& 24.6 / 35.0& 41.6& 22.9 / 34.6& 52.9& 28.1 / 26.8 \\
(3) + \factonlydpo& \xmark& \checkmark& 40.8& 47.1& 19.8 / 23.9& 48.2& 17.5 / 19.0& 57.9& 20.0 / 15.9 \\
(4) + \fadpo& \checkmark& \checkmark& \textbf{51.7}& 44.9& 23.7 / 30.3& 45.0& 23.1 / 28.7& 56.4 &27.1 / 23.3\\
\hline
 (5) \fasft& -& -& 29.1& \textbf{49.5}& 19.9 / 19.5& 41.4& 18.3 / 27.7& 54.2& 19.3 / 22.4\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
(6) + \dpo&\checkmark & \xmark& 50.4& 46.3& 24.0 /  28.7& 43.9& 21.6 / 28.8& 55.0& 25.4 / 22.0 \\
(7) + \fadpo& \checkmark& \checkmark& 51.2& 47.9& 25.9 / 28.5& \textbf{48.7}& 24.1 / 25.5& \textbf{58.9}& 29.0 / 22.2\\

\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table*}


==> Factuality-Aware_Alignment_For_Large_Language_Models/fact_based_classification_ablations.tex <==
\begin{table}[h]
	\caption{Effects of fact-based classification on factuality-aware alignment.}
	\label{tb:fact_based_classification_ablations}
	\centering
	 \resizebox{1\columnwidth}{!}{ 
  \begin{threeparttable}
	  \setlength\tabcolsep{0.05cm}
    \begin{tabular}{ll|cc|c|ccc}
\hline \hline

&&  \multicolumn{2}{c}{Classifier}&\multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{\textbf{Bio}}}\\
 \cmidrule(rl){3-4} \cmidrule(rl){5-5} \cmidrule(rl){6-7}
&& Inst.& Sent.& win rate& FS& \# Corr. / Err.\\
 \hline
(1)&\multirow{2}{*}{\fasft}& \xmark& -& 47.6\tnote{$\ast$}& 48.4& 20.5 / 21.4\\
(2)&&\checkmark & -&51.2\tnote{$\ast$}&49.5& 19.9 / 19.5 \\
\hline
(3)&\multirow{3}{*}{\sft\ + \fadpo}& \xmark& \xmark& 46.8\tnote{$\triangle$}& 46.8& 21.7 / 25.3\\
(4)&&\checkmark & \xmark&51.7\tnote{$\triangle$}& 45.0& 23.7 / 30.3 \\
% \arrayrulecolor{lightgray}
% \hline
(5)&&\checkmark & \checkmark& 51.3\tnote{$\triangle$}& 42.9& 25.5 / 36.8 \\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
 \begin{tablenotes}
	\item[$\ast$] comparing with SFT baseline, \sft. 
        \item[$\triangle$] comparing with DPO baseline, \sft{} + \dpo. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality-Aware_Alignment_For_Large_Language_Models/factuality_rm_comparison.tex <==
\begin{table}[t!]
	\caption{A comparison of factuality reward models. $\tau$ denotes the correlation between human annotation.}
	\label{tb:factuality_rm_comparison}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	   % \setlength\tabcolsep{0.05cm}
    \begin{tabular}{clccc}
\hline \hline
 & fact check model& \# sup.& fact unit& $\tau$\\
 \hline
 (1)& \multirow{2}{*}{Instruct Llama 7B}& 5& \multirow{2}{*}{atom.}& 0.32\\
 (2)& & 10& & 0.34\\
  \hline
 (3)& \multirow{2}{*}{\sft\ (Llama-2 70B)}& 5& \multirow{2}{*}{atom.}& 0.28\\
 (4)& & 10& & 0.31\\
 \hline
 (5)& \multirow{2}{*}{Instruct Llama 7B}& 5& \multirow{2}{*}{sent.}& 0.20\\
 (6)& & 10& & 0.25\\
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}


==> Factuality-Aware_Alignment_For_Large_Language_Models/impacts_of_response_length.tex <==
\begin{table}[t!]
	\caption{Effects of DPO training on response length.}
	\label{tb:impact_of_dpo_finetuning_on_generation_length}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|c|c|c|c}
\hline \hline
& \textbf{Alpaca Eval}& \textbf{Bio}& \textbf{Alpaca Fact}& \textbf{FAVA}\\
 \hline
 (1) \sft& \ \ 897&	1221& \ \ 969& \ \ 912\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
 (2) + \dpo& 1470&	1494& 1586& 1540\\
 (3) + \factonlydpo& 1160&	1166& 1192& 1104\\
 (4) + \fadpo& 1474&	1395& 1528& 1422\\

\arrayrulecolor{black}
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}


==> Factuality-Aware_Alignment_For_Large_Language_Models/sft_exp.tex <==
\begin{table*}[t!]
	\caption{Experimental results of supervised fine-tuning on Open Assistant dataset. \pt{} denotes pre-trained Llama2 70B with 5-shot demonstration. \factonlysft{} denotes the variant which only optimizes factuality. FS denotes FActScore.}
	\label{tb:main_sft_results}
	\centering
	 \resizebox{1\textwidth}{!}{  
  \begin{threeparttable}
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|cc|c|cc|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 70B}& \multicolumn{2}{c}{src. of supervision}& \multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{\textbf{Bio}}}&\multicolumn{2}{c}{\textbf{Alpaca Fact}}& \multicolumn{2}{c}{\textbf{FAVA}}\\
\cmidrule(rl){2-3} \cmidrule(rl){4-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(rl){9-10}      
& \human& \pt& win rate over (1)& FS& \# Corr. / Err.& FS& \# Corr. / Err.& FS& \# Corr. / Err.\\
 \hline
 (0) \pt& -& -& -& 53.1& 15.3 / 13.5& -& -& -& -\\
 \hline
 (1) \sft& \checkmark& \xmark& 50.0& 44.7& 21.1 / 26.8& 38.6& 16.7 / 29.0& \textbf{54.4}& 21.2 / 25.8\\
 (2) \factonlysft& \xmark& \checkmark& 48.1& 48.5& 19.6 / 20.6& \textbf{42.0}& 17.5 / 28.4& 53.3& 18.3 / 24.2\\
 (3) \fasft& \checkmark\tnote{$\ast$}& \checkmark\tnote{$\ast$}& \textbf{51.2}& \textbf{49.5}& 19.9 / 19.5& 41.4& 18.3 / 27.7& 54.2& 19.3 / 22.4\\

\arrayrulecolor{black}
\hline \hline
	\end{tabular}
\begin{tablenotes}
	\item[$\ast$] \fasft{} uses supervision from \human{} and \pt{} for non-fact-based and fact-based instructions, respectively. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table*}


==> Factuality-Aware_Alignment_For_Large_Language_Models/training_data_statistics.tex <==
\begin{table}[t]
	\caption{Training data statistics for different variants. IF.~and Fact.~denote instruction following $(x, y_{+}, y_{-})$ and factuality $(x \in X^{\text{\tiny fact}}, y_{\text{\tiny true}}, y_{\text{\tiny false}})$ preference data, where $X^{\text{\tiny fact}}$ denotes the set of fact-based instructions.}
	\label{tb:training_data_statistics}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
& \multicolumn{2}{c}{\textbf{Seed IFT (\# of Inst.)}}& \multicolumn{2}{c}{\textbf{Preference (\# of pairs)}}\\
  \cmidrule(rl){2-3} \cmidrule(rl){4-5}
model variant&$x \notin X^{\text{\tiny fact}}$ & $x \in X^{\text{\tiny fact}}$&IF. & Fact.\\
\hline
\sft\ + \dpo& \multirow{3}{*}{2,187}& \multirow{3}{*}{1,013}& 18,454& - \\ 
\sft\ + \factonlydpo& & & -& 3,315\\ 
\sft\ + \fadpo& & & 18,454& 3,315\\ 
\hline
\fasft\ + \dpo& \multirow{2}{*}{2,187}& \multirow{2}{*}{1,013}& 18,603& - \\ 
\fasft\ + \fadpo& & & 18,603& 4,211 \\ 
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality-Aware_Alignment_For_Large_Language_Models/truthfulqa.tex <==
\begin{table}[t!]
	\caption{Results on TruthfulQA.}
	\label{tb:truthfulqa}
	\centering
	 \resizebox{0.95\columnwidth}{!}{  
	  \setlength\tabcolsep{0.14cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
 \multirow{2}{*}{Llama-2 70B} & \multicolumn{2}{c|}{src. of supervision}& \multicolumn{2}{c}{\textbf{TruthfulQA}}\\
  \cmidrule(rl){2-3}  \cmidrule(rl){4-5}
 & IF.& Fact.& BLUE & ROUGE \\
 \hline
 (0) Chat& \multicolumn{2}{c|}{Proprietary data}& 0.21& 1.16\\
 \hline
 (1) \sft& -& -& 0.37& 0.20\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
  (2) + \dpo& \checkmark& \xmark& 0.03& 0.54\\
 (3) + \factonlydpo& \xmark& \checkmark& 0.30& 1.12\\
 (4) + \fadpo& \checkmark& \checkmark& 0.15&	0.80\\
 \hline
 (5) \fasft& -& -& 0.39& 0.51\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
 (6) + \dpo& \checkmark& \xmark&0.07& 0.91\\
 (7) + \fadpo& \checkmark& \checkmark& 0.20& 0.96\\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}


==> Factuality_Aware_Alignment_For_Large_Language_Models/bio_gen_exp.tex <==
\begin{table}[t!]
	\caption{Pilot study on biography generation. Pos. denotes the positives for SFT or DPO. Neg. denotes the negatives for DPO. FS denotes FActScore.}
	\label{tb:pilot_study_bio_gen}
	\centering
	 \resizebox{1\columnwidth}{!}{  
   \begin{threeparttable}
	  % \setlength\tabcolsep{0.2cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 7B}& \multicolumn{2}{c|}{src. of supervision}& \multicolumn{2}{c}{\textbf{Bio}} \\
\cmidrule(rl){2-3} \cmidrule(rl){4-5} 
 & Pos.& Neg.& FS& \# Corr. / Err.\\
 \hline
 % (1)& Chat version&	32.4&	21.3&	43.4 \\
 (1) \pt& -& -&	39.1&	14.4 / 22.0\\
 (2) \ragpt& -& -&55.4&	18.6 / 15.9\\
 \hline
(3) \multirow{2}{*}{\sft} & \pt& -&	37.9&	13.4 / 21.8\\
(4) & \ragpt& -&	35.7&	13.5 / 23.7\\
 \hline
(5) \multirow{2}{*}{\dpo} & \pt\tnote{$\ast$}& \pt\tnote{$\ast$}&	41.6&	15.4 / 20.7\\
(6) & \ragpt& \pt&	23.5& 12.7 / 34.9\\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
 		\begin{tablenotes}
	\item[$\ast$] FActScore is used to select positives and negatives. 
    \end{tablenotes}
    \end{threeparttable}
	}
 \vspace{-0.4cm}
\end{table}


==> Factuality_Aware_Alignment_For_Large_Language_Models/dpo_ablation.tex <==
\begin{table}[t]
	\caption{Ablation on factuality preference data creation.}
	\label{tb:dpo_ablations}
	\centering
	 \resizebox{1\columnwidth}{!}{  
\begin{threeparttable}
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{ccc|c|c}
\hline \hline
\multicolumn{3}{c|}{Factuality preference data}&\multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{1}{c}{\textbf{\textbf{Bio}}}\\
 \cmidrule(rl){1-3} \cmidrule(rl){4-4} \cmidrule(rl){5-5}
Reward model& Pos.,Neg.& \# pairs& win rate\tnote{$\triangle$}& FS\\
\hline
\factrm& max, min& 3,315& 51.7& 44.9\\
\factrm& enum.& 5,126& 50.7& 45.0\\
\selfrm\ + $5*$\factrm& max, min& 6,340& 50.1& 45.1 \\
\hline \hline
	\end{tabular}
 \begin{tablenotes}
        \item[$\triangle$] comparing with DPO baseline, \sft{} + \dpo. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality_Aware_Alignment_For_Large_Language_Models/dpo_exp.tex <==
\begin{table*}[t!]
\caption{Experiments of direct preference optimization (DPO). IF.~and Fact.~denote instruction following $(x, y_{+}, y_{-})$ and factuality $(x \in X^{\text{\tiny fact}}, y_{\text{\tiny true}}, y_{\text{\tiny false}})$ preference data, where $X^{\text{\tiny fact}}$ denotes the set of fact-based instructions. \factonlydpo{} denotes the variant which only optimizes factuality. The preference data statistics is listed in Appendix, Table~\ref{tb:training_data_statistics}.}
	\label{tb:main_dpo_results}
	\centering
	 \resizebox{1\textwidth}{!}{  
	  % \setlength\tabcolsep{0.15cm}
    \begin{tabular}{l|cc|c|cc|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 70B} & \multicolumn{2}{c|}{src. of supervision}& \multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{Bio}}& \multicolumn{2}{c}{\textbf{Alpaca Fact}}& \multicolumn{2}{c}{\textbf{FAVA}}\\
 \cmidrule(rl){2-3} \cmidrule(rl){4-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(rl){9-10}
 & IF.& Fact.& win rate over  (2)& FS& \# Corr. / Err.& FS& \# Corr. / Err.& FS& \# Corr. / Err.\\
 \hline
 (0) Chat& \multicolumn{2}{c|}{Proprietary data}& 66.2& 33.2& 23.4 / 43.6& 39.3& 22.3 / 36.4& 47.5& 28.0 / 31.3\\
 \hline
 (1) \sft& -& -& 27.1& 44.7& 21.1 / 26.8& 38.6& 16.7 / 29.0& 54.4& 21.2 / 25.8\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
(2) + \dpo& \checkmark& \xmark& 50.0& 42.3& 24.6 / 35.0& 41.6& 22.9 / 34.6& 52.9& 28.1 / 26.8 \\
(3) + \factonlydpo& \xmark& \checkmark& 40.8& 47.1& 19.8 / 23.9& 48.2& 17.5 / 19.0& 57.9& 20.0 / 15.9 \\
(4) + \fadpo& \checkmark& \checkmark& \textbf{51.7}& 44.9& 23.7 / 30.3& 45.0& 23.1 / 28.7& 56.4 &27.1 / 23.3\\
\hline
 (5) \fasft& -& -& 29.1& \textbf{49.5}& 19.9 / 19.5& 41.4& 18.3 / 27.7& 54.2& 19.3 / 22.4\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
(6) + \dpo&\checkmark & \xmark& 50.4& 46.3& 24.0 /  28.7& 43.9& 21.6 / 28.8& 55.0& 25.4 / 22.0 \\
(7) + \fadpo& \checkmark& \checkmark& 51.2& 47.9& 25.9 / 28.5& \textbf{48.7}& 24.1 / 25.5& \textbf{58.9}& 29.0 / 22.2\\

\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table*}


==> Factuality_Aware_Alignment_For_Large_Language_Models/fact_based_classification_ablations.tex <==
\begin{table}[h]
	\caption{Effects of fact-based classification on factuality-aware alignment.}
	\label{tb:fact_based_classification_ablations}
	\centering
	 \resizebox{1\columnwidth}{!}{ 
  \begin{threeparttable}
	  \setlength\tabcolsep{0.05cm}
    \begin{tabular}{ll|cc|c|ccc}
\hline \hline

&&  \multicolumn{2}{c}{Classifier}&\multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{\textbf{Bio}}}\\
 \cmidrule(rl){3-4} \cmidrule(rl){5-5} \cmidrule(rl){6-7}
&& Inst.& Sent.& win rate& FS& \# Corr. / Err.\\
 \hline
(1)&\multirow{2}{*}{\fasft}& \xmark& -& 47.6\tnote{$\ast$}& 48.4& 20.5 / 21.4\\
(2)&&\checkmark & -&51.2\tnote{$\ast$}&49.5& 19.9 / 19.5 \\
\hline
(3)&\multirow{3}{*}{\sft\ + \fadpo}& \xmark& \xmark& 46.8\tnote{$\triangle$}& 46.8& 21.7 / 25.3\\
(4)&&\checkmark & \xmark&51.7\tnote{$\triangle$}& 45.0& 23.7 / 30.3 \\
% \arrayrulecolor{lightgray}
% \hline
(5)&&\checkmark & \checkmark& 51.3\tnote{$\triangle$}& 42.9& 25.5 / 36.8 \\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
 \begin{tablenotes}
	\item[$\ast$] comparing with SFT baseline, \sft. 
        \item[$\triangle$] comparing with DPO baseline, \sft{} + \dpo. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality_Aware_Alignment_For_Large_Language_Models/factuality_rm_comparison.tex <==
\begin{table}[t!]
	\caption{A comparison of factuality reward models. $\tau$ denotes the correlation between human annotation.}
	\label{tb:factuality_rm_comparison}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	   % \setlength\tabcolsep{0.05cm}
    \begin{tabular}{clccc}
\hline \hline
 & fact check model& \# sup.& fact unit& $\tau$\\
 \hline
 (1)& \multirow{2}{*}{Instruct Llama 7B}& 5& \multirow{2}{*}{atom.}& 0.32\\
 (2)& & 10& & 0.34\\
  \hline
 (3)& \multirow{2}{*}{\sft\ (Llama-2 70B)}& 5& \multirow{2}{*}{atom.}& 0.28\\
 (4)& & 10& & 0.31\\
 \hline
 (5)& \multirow{2}{*}{Instruct Llama 7B}& 5& \multirow{2}{*}{sent.}& 0.20\\
 (6)& & 10& & 0.25\\
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}


==> Factuality_Aware_Alignment_For_Large_Language_Models/impacts_of_response_length.tex <==
\begin{table}[t!]
	\caption{Effects of DPO training on response length.}
	\label{tb:impact_of_dpo_finetuning_on_generation_length}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|c|c|c|c}
\hline \hline
& \textbf{Alpaca Eval}& \textbf{Bio}& \textbf{Alpaca Fact}& \textbf{FAVA}\\
 \hline
 (1) \sft& \ \ 897&	1221& \ \ 969& \ \ 912\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
 (2) + \dpo& 1470&	1494& 1586& 1540\\
 (3) + \factonlydpo& 1160&	1166& 1192& 1104\\
 (4) + \fadpo& 1474&	1395& 1528& 1422\\

\arrayrulecolor{black}
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}


==> Factuality_Aware_Alignment_For_Large_Language_Models/sft_exp.tex <==
\begin{table*}[t!]
	\caption{Experimental results of supervised fine-tuning on Open Assistant dataset. \pt{} denotes pre-trained Llama2 70B with 5-shot demonstration. \factonlysft{} denotes the variant which only optimizes factuality. FS denotes FActScore.}
	\label{tb:main_sft_results}
	\centering
	 \resizebox{1\textwidth}{!}{  
  \begin{threeparttable}
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|cc|c|cc|cc|cc}
\hline \hline
\multirow{2}{*}{Llama-2 70B}& \multicolumn{2}{c}{src. of supervision}& \multicolumn{1}{c}{\textbf{Alpaca Eval}}& \multicolumn{2}{c}{\textbf{\textbf{Bio}}}&\multicolumn{2}{c}{\textbf{Alpaca Fact}}& \multicolumn{2}{c}{\textbf{FAVA}}\\
\cmidrule(rl){2-3} \cmidrule(rl){4-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8} \cmidrule(rl){9-10}      
& \human& \pt& win rate over (1)& FS& \# Corr. / Err.& FS& \# Corr. / Err.& FS& \# Corr. / Err.\\
 \hline
 (0) \pt& -& -& -& 53.1& 15.3 / 13.5& -& -& -& -\\
 \hline
 (1) \sft& \checkmark& \xmark& 50.0& 44.7& 21.1 / 26.8& 38.6& 16.7 / 29.0& \textbf{54.4}& 21.2 / 25.8\\
 (2) \factonlysft& \xmark& \checkmark& 48.1& 48.5& 19.6 / 20.6& \textbf{42.0}& 17.5 / 28.4& 53.3& 18.3 / 24.2\\
 (3) \fasft& \checkmark\tnote{$\ast$}& \checkmark\tnote{$\ast$}& \textbf{51.2}& \textbf{49.5}& 19.9 / 19.5& 41.4& 18.3 / 27.7& 54.2& 19.3 / 22.4\\

\arrayrulecolor{black}
\hline \hline
	\end{tabular}
\begin{tablenotes}
	\item[$\ast$] \fasft{} uses supervision from \human{} and \pt{} for non-fact-based and fact-based instructions, respectively. 
    \end{tablenotes}
    \end{threeparttable}
	}
 % \vspace{-0.2cm}
\end{table*}


==> Factuality_Aware_Alignment_For_Large_Language_Models/training_data_statistics.tex <==
\begin{table}[t]
	\caption{Training data statistics for different variants. IF.~and Fact.~denote instruction following $(x, y_{+}, y_{-})$ and factuality $(x \in X^{\text{\tiny fact}}, y_{\text{\tiny true}}, y_{\text{\tiny false}})$ preference data, where $X^{\text{\tiny fact}}$ denotes the set of fact-based instructions.}
	\label{tb:training_data_statistics}
	\centering
	 \resizebox{1\columnwidth}{!}{  
	  % \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
& \multicolumn{2}{c}{\textbf{Seed IFT (\# of Inst.)}}& \multicolumn{2}{c}{\textbf{Preference (\# of pairs)}}\\
  \cmidrule(rl){2-3} \cmidrule(rl){4-5}
model variant&$x \notin X^{\text{\tiny fact}}$ & $x \in X^{\text{\tiny fact}}$&IF. & Fact.\\
\hline
\sft\ + \dpo& \multirow{3}{*}{2,187}& \multirow{3}{*}{1,013}& 18,454& - \\ 
\sft\ + \factonlydpo& & & -& 3,315\\ 
\sft\ + \fadpo& & & 18,454& 3,315\\ 
\hline
\fasft\ + \dpo& \multirow{2}{*}{2,187}& \multirow{2}{*}{1,013}& 18,603& - \\ 
\fasft\ + \fadpo& & & 18,603& 4,211 \\ 
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}

==> Factuality_Aware_Alignment_For_Large_Language_Models/truthfulqa.tex <==
\begin{table}[t!]
	\caption{Results on TruthfulQA.}
	\label{tb:truthfulqa}
	\centering
	 \resizebox{0.95\columnwidth}{!}{  
	  \setlength\tabcolsep{0.14cm}
    \begin{tabular}{l|cc|cc}
\hline \hline
 \multirow{2}{*}{Llama-2 70B} & \multicolumn{2}{c|}{src. of supervision}& \multicolumn{2}{c}{\textbf{TruthfulQA}}\\
  \cmidrule(rl){2-3}  \cmidrule(rl){4-5}
 & IF.& Fact.& BLUE & ROUGE \\
 \hline
 (0) Chat& \multicolumn{2}{c|}{Proprietary data}& 0.21& 1.16\\
 \hline
 (1) \sft& -& -& 0.37& 0.20\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
  (2) + \dpo& \checkmark& \xmark& 0.03& 0.54\\
 (3) + \factonlydpo& \xmark& \checkmark& 0.30& 1.12\\
 (4) + \fadpo& \checkmark& \checkmark& 0.15&	0.80\\
 \hline
 (5) \fasft& -& -& 0.39& 0.51\\
 \arrayrulecolor{lightgray}
 \hline
 \arrayrulecolor{black}
 (6) + \dpo& \checkmark& \xmark&0.07& 0.91\\
 (7) + \fadpo& \checkmark& \checkmark& 0.20& 0.96\\
\arrayrulecolor{black}
\hline \hline
	\end{tabular}
	}
 % \vspace{-0.2cm}
\end{table}

